Scaling Vision Transformers to Gigapixel Images via Hierarchical Self-Supervised Learning

Vision Transformers (ViTs) and their multi-scale and hierarchical variations have been successful at capturing image representations but their use has been generally studied for low-resolution images (e.g. - 256x256, 384384). For gigapixel whole-slide imaging (WSI) in computational pathology, WSIs can be as large as 150000x150000 pixels at 20X magnification and exhibit a hierarchical structure of visual tokens across varying resolutions: from 16x16 images capture spatial patterns among cells, to 4096x4096 images characterizing interactions within the tissue microenvironment. We introduce a new ViT architecture called the Hierarchical Image Pyramid Transformer (HIPT), which leverages the natural hierarchical structure inherent in WSIs using two levels of self-supervised learning to learn high-resolution image representations. HIPT is pretrained across 33 cancer types using 10,678 gigapixel WSIs, 408,218 4096x4096 images, and 104M 256x256 images. We benchmark HIPT representations on 9 slide-level tasks, and demonstrate that: 1) HIPT with hierarchical pretraining outperforms current state-of-the-art methods for cancer subtyping and survival prediction, 2) self-supervised ViTs are able to model important inductive biases about the hierarchical structure of phenotypes in the tumor microenvironment.

==> fig/attention.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\linewidth]{FigX_Attention1.jpg}
\end{center}
\caption{\textbf{Multi-Head Self-Attention Visualization of Self-Supervised ViTs}. We show attention visualizations for VIT-16 (trained on $\textbf{x}_{256}$ patches) and VIT-256 (trained on $\textbf{x}_{4096}$ regions). \textbf{Left. Invasive Ductal Carcinoma (IDC).} For $\textbf{x}_{256}$ patches, ViT-16 is able to delineate stroma, cell, and "white space" presence in $\textbf{x}_{16}$ tokens. From ViT-256, we observe disentanglement of coarse-grained morphological features such as tumor nests and their surrounding desmoplastic (loose) stroma. \textbf{Right. Colorectal cancer (CRC).} We observe similar delineation of stroma, cells, and "white space" presence in CRC. From ViT-256, we observe different attention heads localizing poorly-differentiated glands, as well as tumor invasion into muscle.}
\label{fig:attention1}
\end{figure*}

==> fig/attention2.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=.99\linewidth]{Fig3_Attention2.jpg}
\end{center}
\caption{\small\textbf{Multi-Head Self-Attention Visualization of Self-Supervised ViTs}. For Invasive Ductal Carcinoma (IDC), We show self-supervised attention visualizations for VIT-16 (trained on $\textbf{x}_{256}$ patches) and VIT-256 (trained on $\textbf{x}_{4096}$ regions). For $\textbf{x}_{256}$ patches, ViT-16 is able to delineate stroma, cell, and "white space" presence in $\textbf{x}_{16}$ tokens. From ViT-256, we observe disentanglement of coarse-grained morphological features such as tumor nests and their surrounding desmoplastic (loose) stroma.}
\label{fig:attention2}
\end{figure}


==> sec/1_introduction_v1.tex <==
\vspace{-4mm}
\section{Introduction}
\label{sec:intro}
% 
\input{fig/teaser}
% \let\thefootnote\relax\footnote{* Contributed Equally}
Tissue phenotyping is a important problem in computational pathology that aims at characterizing objective, histopathologic biomarkers within the tumor-immune microenvironment for cancer diagnosis, prognosis, and the estimation of response-to-treatment in patients \cite{ludwig2005biomarkers, kather2016multi, javed2020cellular}. 
The current clinical paradigm is the manual and subjective interpretation of histology whole-slide images (WSI) in determining clinical endpoints such as cancer subtype, grade, and stage~\cite{amin2017eighth}. 

The successes of deep learning have found their way to computational histopathology, in which frameworks such as multiple instance learning (MIL) have been used to build predictive models of clinical outcomes using WSI~\cite{hou2016patch, courtiol2019deep, wulczyn2020deep, van2019no, tellez2019neural, ilse2018attention, campanella2019clinical, lu2020data}. Such frameworks follow three steps. First, instance-level patch representations are extracted from non-overlapping tissue patches in the WSI (typically using variations of ResNet models. Second, global pooling is applied over the bag of patches to construct a WSI-level representation which forms the input to different classifiers~\cite{krizhevsky2012imagenet, ilse2018attention}. Finally, a classifier is trained on the WSI-level representation to predict outcomes of interest. 

This three stage process has a few important limitations. First, a pre-trained ResNet model may not capture the right representation of the tumor microenvironment. Second, although clinician annotations are the gold standard in taxonomic classifications and staging systems for many cancer types, they have been demonstrated to suffer from large inter- and intra-observer variability~\cite{nicholson2001reproducibility, rabe2019interobserver, echle2020bjc}. e.g. the substantial variability in discerning well-to-poorly differentiated glands in the Gleason grading system for prostate adenocarcinoma, or the evaluation of nuclear size, shape, and nucleolar prominence in the Furhman grading system for renal cell carcinoma~\cite{carlson1998accuracy, novara2007grading}. Recent work has shown that self-supervised learning can serve as an effective strategy to improve upon the representations learned from a ResNet encoder \emph{without} the use of labels\cite{ciga2021self, saillard2021self, dehaene2020self, koohbanani2021self, boyd2021self, li2021dual}.
In this work, we push the limits of self-supervised learning by leveraging structure inherent to histopathological tissue samples to develop new models and algorithms for self-supervised learning closer to the whole-slide level. 

A pathologist scanning a WSI will scan the sample at multiple different resolutions with each resolution presenting the clinician with information about cellular abnormalities, spatial organization of cells and tissue level phenotypes. 
Figure \ref{fig:hier_wsi} depicts the organization of information at various levels of granularity within a WSI.
WSIs scanned at $20\times$ objective typically use a fixed scale of $0.5 \mu m$ per pixel. This has an important implication: across different WSIs, the fixed scale enables consistent comparison of visual elements that may elucidate important histomorphological features. WSIs also exhibit a hierarchical structure of visual tokens at varying image resolutions at $20\times$ magnification: the $16 \times 16$ images encompass the bounding box of cells and other fine-grained features (stroma, tumor cells, lymphocytes), $256 \times 256$ images capture local clusters of cell-to-cell interactions (tumor cellularity), $1024 \times 1024$-$4096 \times 4096$ images further characterize macro-scale interactions between clusters of cells and their organization in tissue (the extend of tumor-immune localization in describing tumor-infiltrating versus tumor-distal lymphocytes), and finally the overall intra-tumoral heterogeneity of the tissue microenvironment depicted at the slide-level of the WSI~\cite{beck2011systematic, sertel2009histopathological, javed2020cellular, zhu2017wsisa, hou2019sparse, Diao2021, saltz2018spatial}. The hypothesis that this work tests is that the judicious use of this hierarchy in self-supervised learning results in better whole slide level representations. 

%which we note has several shared properties that connect WSIs closer to the language domain than computer vision. Despite the gigapixel image resolutions of WSIs that seemingly make supervision intractable in comparison to $256 \times 256$ natural images, \textbf{\textit{a key difference is that visual tokens in WSIs are always at a fixed scale for a given magnification objective}}. For instance, WSIs scanned at $20\times$ objective have a fixed scale of $0.5 \mu m$ per pixel, which allows for consistent comparison of visual elements that may elucidate important histomorphological features such as nuclear atypia, which describes irregularities in shape and size of cells beyond their normal reference ranges. 
%Despite the natural part-whole hierarchy of histopathology tissue and the varying fine-to-coarse grained semantic information of visual tokens across image resolutions, conventional weakly-supervised approaches based on multiple instance learning (MIL) typically perform patching at the $256 \times 256$-level, with only global pooling applied without self-attention due to the intractable sequence lengths (or bag sizes) of gigapixel WSIs. As a result, MIL approaches typically perform learning on only instance-level features and do not use Transformer attention in learning context-aware relationships between visual tokens. Moreover, tokenization is often performed using a ResNet-50 encoder pretrained on ImageNet, which may not generalize to domain-specific challenges in cancer pathology. While self-supervised learning has emerged as a strategy for pretraining the instance-level feature extraction component of MIL methods, progress towards developing slide-level pretraining approaches remain relatively unexplored.

To operationalize our insight, we introduce a Transformer-based architecture for hierarchical aggregation of visual tokens and pretraining in gigapixel pathology images, called Hierarchical Image Pyramid Transformer (HIPT). We approach the task of slide level representation learning in a manner similar to the construction of representations of documents in language modeling~\cite{yang2016hierarchical, zhang2019hibert}. Specifically, similar to how hierarchical attention networks for long document classification aggregate word embeddings within sentences to form sentence-level embeddings and subsequently into document-level embeddings, we develop a three-stage hierarchical architecture that performs similar bottom-up aggregation from [$16 \times 16$] visual tokens in their respective $256 \times 256$ and $4096 \times 4096$ windows to eventually form the slide-level representation, as demonstrated in Figure \ref{fig:overview}. While patching in WSIs can result in variable sequence lengths, we choose a large image resolution to patch at first ($\textit{e.g.} - [4096 \times 4096$]) so that further patching within these image regions into $[256 \times 256]$ tokens (and subsequently into $[16 \times 
16]$ tokens) would have constant sequence lengths. 
In summary, the key contributions of our work are as follows. 
\begin{enumerate}
    \item We propose the Hierarchical Image Pyramid Transformer (HIPT); a model capable of learning meaningful representations of high-resolution images.
    \item We apply HIPT to the task of learning representations of gigapixel histopathological images extracted at $20\times$ resolution. We show that our method achieves superior performance to conventional MIL approaches. The difference is pronounced in context-aware tasks such as survival prediction in which larger context is appreciated in characterizing broader prognostic features in the tumor microenvironment~\cite{thorsson2018immune, saltz2018spatial, abduljabbar2020geospatial, chen2021multimodal}. Using K-Nearest Neighbors on the $4096 \times 4096$ representations of our model, we outperform several weakly-supervised architectures in slide-level classification -- an important step forward in achieving self-supervised slide-level representations.
    \item Akin to self-supervised ViTs on natural images that encode semantic segmentation of the scene layout, we find that the multi-head self-attention in self-supervised ViTs learns \emph{disentagled} representations of histology images as unique visual concepts (from fine-grained visual concepts such as cell locations in the $\operatorname{ViT-16}$ to coarse-grained visual concepts such as broader tumor cellularity in the $\operatorname{ViT-256}$), as demonstrated in Figure \ref{fig:attention1}. 
    \item We make all code and pretrained weights publicly available at \href{https://github.com/707884/707884}{https://github.com/707884/707884}.
\end{enumerate}
%As a result, the effect of our network design is two-fold: 

%\begin{enumerate}
%    \item First, we can tractably extend self-attention computation in modeling interactions between tokens at each layer of the hierarchy. For $[16 \times 16]$ cell aggregation, $[256 \times 256]$ patch aggregation and $4096 \times 4096$ region aggregation, we use three vanilla ViT backbones (denoted as $\operatorname{ViT-16}$, $\operatorname{ViT-256}$, $\operatorname{ViT-4096}$ respectively).
    % Features extracted from the $\operatorname{ViT-16}$ (with $16 \times 16$ patching) are used as visual tokens for the $\operatorname{ViT-256}$.
%\item In using Transformer attention on fixed image windows, we can also adopt self-supervised ViT techniques for pretraining the self-attention layers in across the different stages of HIPT, in which only the final aggregation layer would need to be finetuned. Specifically, in addition to pretraining a regular $\operatorname{ViT-16}$ using student-teacher knowledge distillation, we also pretrain the $\operatorname{ViT-256}$ using tokens from the $\operatorname{ViT-16}$, denoted as hierarchical pretraining, which can be used to initialize the weights of HIPT. In contrast with conventional weakly-supervised approaches in WSIs that have viewed instance-level tokenization and slide-level aggregation as separate components, the HIPT architecture presents a unified strategy in pretraining the weights of the aggregation layers in MIL frameworks.
%\end{enumerate}

%In our experimentation, we demonstrate that the proposed HIPT architecture achieves strong performance on slide-level cancer classification and survival outcome prediction tasks across a variety of cancer types. Using hierarchical pretraining, we demonstrate that pretraining $16 \times 16$ cell- and $256 \times 256$ patch-level aggregation layers in HIPT is able to achieve superior performance to  conventional MIL approaches, especially in context-aware tasks such as survival prediction in which larger context is appreciated in characterizing broader prognostic features in the tumor microenvironment. Moreover, we demonstrate using simple K-Nearest Neighbors on mean $4096 \times 4096$ embedding from hierarchical pretraining is able to outperform some weakly-supervised architectures in slide-level classification, which we believe is an important step forward in achieving self-supervised slide-level representations.

%Lastly, in performing pretraining, whereas self-supervised ViTs on natural images encode semantic segmentation of the scene layout, we also make the finding that the multi-head self-attention in self-supervised ViTs in the setting of histopathology learns "disentangled" representations of histology images as unique visual concepts (from fine-grained visual concepts such as cell locations in the $\operatorname{ViT-16}$ to coarse-grained visual concepts such as broader tumor cellularity in the $\operatorname{ViT-256}$), as demonstrated in Figure \ref{fig:attention1}. We make all code and pretrained weights publicly available at \href{https://github.com/707884/707884}{https://github.com/707884/707884}.

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
